Proton Irradiation of SiPM arrays for POLAR-2

POLAR-2 is a space-borne polarimeter, built to investigate the polarization of Gamma-Ray Bursts and help elucidate their mechanisms. The instrument is targeted for launch in 2024 or 2025 aboard the China Space Station and is being developed by a collaboration between institutes from Switzerland, Germany, Poland and China. The instrument will orbit at altitudes between 340km and 450km with an inclination of 42$^{\circ}$ and will be subjected to background radiation from cosmic rays and solar events. It is therefore pertinent to better understand the performance of sensitive devices under space-like conditions. In this paper we focus on the radiation damage of the silicon photomultiplier arrays S13361-6075NE-04 and S14161-6050HS-04 from Hamamatsu. The S13361 are irradiated with 58MeV protons at several doses up to 4.96Gy, whereas the newer series S14161 are irradiated at doses of 0.254Gy and 2.31Gy. Their respective performance degradation due to radiation damage are discussed. The equivalent exposure time in space for silicon photomultipliers inside POLAR-2 with a dose of 4.96Gy is 62.9 years (or 1.78 years when disregarding the shielding from the instrument). Primary characteristics of the I-V curves are an increase in the dark current and dark counts, mostly through cross-talk events. Annealing processes at $25^{\circ}C$ were observed but not studied in further detail. Biasing channels while being irradiated have not resulted in any significant impact. Activation analyses showed a dominant contribution of $\beta^{+}$ particles around 511keV. These resulted primarily from copper and carbon, mostly with decay times shorter than the orbital period.

==> Response_to_referee.tex <==


We would like to thank the referee for the detailed comments on the manuscript. We agree with almost all the comments and believe they will help to improve the work. We provide a reply to each of the comments below:

Major comments:

1) Regarding the request for a discussion on the temperature management of the SiPMs we agree that this could be useful to the reader and as such added the following text to page 6 of the manuscript:
 
 "The dark noise rate is proportional to the SiPM temperature. As such, great care was taken in the POLAR-2 design to minimize the temperature of the SiPM arrays. Based on current thermal simulations the mean temperature, as measured on in he centre of each SiPM array, is predicted to be $-10C^\circ$. This is achieved both by providing a good thermal contact to the radiators of the POLAR-2 instrument, through copper pipes, as well as by using a Peltier element directly connected to the SiPM. The Peltier element not only cools the SiPM array by several degrees, it also allows to stabilize the temperature of the SiPMs, during an orbit, to within several degrees through an active control system. This system is based on a PT100 sensor placed on the SiPMs, readout by an FPGA on the front-end electronics which in turn controls the current to the Peltier element. In addition, the bias voltage of the SiPM is controlled by the FPGA in a similar fashion using the input from the PT100 sensor.This allows for a constant gain the SiPM during the mission."
 
2) "Another rcomment is that the supplementary information  the template from the journal for th paper and a number of pictures, but I could not find the pdf of the supplementary information resulting. I suggest - if needed - to include a pdf with the text and captions to figures that you want to include as suppl. Infom"

This comment is unclear to us. We have not included any additional supplementary information like pictures, etc. beyond the main article. If needed we are ready to perform additional correction after more detailed explanation. We refer to: https://www.springer.com/journal/10686/submission-guidelines#Instructions%20for%20Authors_Supplementary%20Information%20(SI)

Minor Comments:

- "P. 1 abstact, Altitude of the CSS is now 425km not 300"
At the start of the analysis, the anticipated altitude of the CSS was unknown. We therefore based our analysis on an educated guess (through our experience of the TG-2). An altitude of 425km is a bit high as well as current live telemetry indicate that it is somewhere around 380km. This may change again. For a more complete picture, we have rerun the simulations to provide annual dose at 340km (low end), 383km (typical) and 450km (high).
You may notice that the dose rate at 300km seems higher than at 340km. However, this results from several updates to the instrument (primarily to the module base to account the mechanical structure for cooling the FEE). A rerun of the sims at 300km shows that the expected dose is \SI{0.0161}{Gy/yr} (before was \SI{0.0638}{Gy/yr}) for the 'Full Instrument + CSS' scenario. The 'typical' altitude of 383km is used to convert from dose to space equivalent years.

- "P2 par 2 The scientific benefits through -- > benefits of gamma-ray polarization studies"
corrected 

- "P2 par 2   [7]. The latter  --> [7], which is the …."
corrected

- " P2 last line will orbit -->  is orbiting "
corrected

 - "P3 line 2 cosmic rays ans solar flare -- > cosmic rays of galactic, solar and trapped origin"
 corrected
 
- "P4 fig1. Very nice fig but it would help if you order the panels in a, c, b and show where each element goes in the other elements. Also c) is upside down in respect to b? a few lines showing the relationship between parts (as in fig 2) would help "
I have rearranged it now as b, c, a. That way we start from the full instrument and end with the scintillator. The module is now aligned with the instrument. I do not think that arrows will be necessary now. 

- "P2 par 2 The scientific benefits through -- > benefits of gamma-ray polarization studies"
agreed and changed

- "P7 a) captions in figure should tell that the non-spenvis is due to leobackground. b)  is very crowded and difficult to discriminate the sources. Perhaps it could be split in two separate figs (also positrons and electrons could go together). Also galactic center and disk should tell that it is gammas from the centre and maybe show them in a thicker line since this is the signal you are looking for"
The captions and/or legends have been adjusted and the figures have been split to avoid a crowded representation. I wouldn't put electrons and positrons together to maintain the integrity of the tool used to generate them. 

- "P7 sect 3 explain in a couple of lines what is the SAA
P7 l10 spenvis only provides information on TRAPPED protons…."
indeed. updated

- "P7 “accounting for… their flux… “ it better to rephrase: “flux of trapper particles in the SAA is at least”"
corrected

- "P12 third paragraph line l8 temperate -- > temperature"
corrected

- "p12 l12   …at the SIPM output. change of about…. The two phrases are disjoint"
fixed

- "P15 first bullet add a reference to the Saviztky-golay filter"
done

- "Fig 12-19 (except 15) should mention the Z axis scale (color scale) on the Amplitude-Deltat colour Z plots (at least in the caption, since redoing all pics  for the Z axis can be troublesome)"
done

- "P28 we present -- > have presented"
done

- "P28 par 2 last line what is close -- > that is close"
done



==> sn-sample-bib.tex <==
\begin{thebibliography}{9}



\end{thebibliography}


